The Complexity of Constrained Min-Max Optimization

Despite its important applications in Machine Learning, min-max optimization of nonconvex-nonconcave objectives remains elusive. Not only are there no known first-order methods converging even to approximate local min-max points, but the computational complexity of identifying them is also poorly understood. In this paper, we provide a characterization of the computational complexity of the problem, as well as of the limitations of first-order methods in constrained min-max optimization problems with nonconvex-nonconcave objectives and linear constraints. As a warm-up, we show that, even when the objective is a Lipschitz and smooth differentiable function, deciding whether a min-max point exists, in fact even deciding whether an approximate min-max point exists, is NP-hard. More importantly, we show that an approximate local min-max point of large enough approximation is guaranteed to exist, but finding one such point is PPAD-complete. The same is true of computing an approximate fixed point of Gradient Descent/Ascent. An important byproduct of our proof is to establish an unconditional hardness result in the Nemirovsky-Yudin model. We show that, given oracle access to some function $f : P \to [-1, 1]$ and its gradient $\nabla f$, where $P \subseteq [0, 1]^d$ is a known convex polytope, every algorithm that finds a $\varepsilon$-approximate local min-max point needs to make a number of queries that is exponential in at least one of $1/\varepsilon$, $L$, $G$, or $d$, where $L$ and $G$ are respectively the smoothness and Lipschitzness of $f$ and $d$ is the dimension. This comes in sharp contrast to minimization problems, where finding approximate local minima in the same setting can be done with Projected Gradient Descent using $O(L/\varepsilon)$ many queries. Our result is the first to show an exponential separation between these two fundamental optimization problems.

==> Local min max/headers/bbhead.tex <==
% blackboard symbols

\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\D}{\ensuremath{\mathbb{D}}}
\newcommand{\F}{\ensuremath{\mathbb{F}}}
\newcommand{\G}{\ensuremath{\mathbb{G}}}
%\newcommand{\J}{\ensuremath{\mathbb{J}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\T}{\ensuremath{\mathbb{T}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}

\newcommand{\Zt}{\ensuremath{\Z_t}}
\newcommand{\Zp}{\ensuremath{\Z_p}}
\newcommand{\Zq}{\ensuremath{\Z_q}}
\newcommand{\ZN}{\ensuremath{\Z_N}}
\newcommand{\Zps}{\ensuremath{\Z_p^*}}
\newcommand{\ZNs}{\ensuremath{\Z_N^*}}
\newcommand{\JN}{\ensuremath{\J_N}}
\newcommand{\QRN}{\ensuremath{\mathbb{QR}_N}}
\newcommand{\Fq}{\ensuremath{\F_q}}


==> Local min max/headers/calhead.tex <==
% hash functions
\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calJ}{\ensuremath{\mathcal{J}}}
\newcommand{\calK}{\ensuremath{\mathcal{K}}}
\newcommand{\calL}{\ensuremath{\mathcal{L}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calO}{\ensuremath{\mathcal{O}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
\newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calW}{\ensuremath{\mathcal{W}}}
\newcommand{\calX}{\ensuremath{\mathcal{X}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\calZ}{\ensuremath{\mathcal{Z}}}

% \newcommand{\calH}{\ensuremath{\mathcal{H}}}
% \newcommand{\calR}{\ensuremath{\mathcal{R}}}
% \newcommand{\calX}{\ensuremath{\mathcal{X}}}
% \newcommand{\calY}{\ensuremath{\mathcal{Y}}}

==> Local min max/headers/comphead.tex <==
% GENERAL COMPUTING STUFF

\newcommand{\bit}{\ensuremath{\set{0,1}}}
\newcommand{\pmone}{\ensuremath{\set{-1,1}}}

% asymptotic stuff
%\DeclareMathOperator{\poly}{poly}
%\DeclareMathOperator{\polylog}{polylog}
\DeclareMathOperator{\negl}{negl}
\newcommand{\Otil}{\ensuremath{\tilde{O}}}

% assorted
\DeclareMathOperator*{\wt}{wt}

\newcommand{\compind}{\ensuremath{\stackrel{c}{\approx}}}
\newcommand{\statind}{\ensuremath{\stackrel{s}{\approx}}}
\newcommand{\perfind}{\ensuremath{\equiv}}

% font for general-purpose algorithms
\newcommand{\algo}[1]{\ensuremath{\mathsf{#1}}\xspace}

% font for general-purpose computational problems
\newcommand{\problem}[1]{\ensuremath{\mathsf{#1}}\xspace}

% font for complexity classes
\newcommand{\class}[1]{\ensuremath{\mathsf{#1}}\xspace}

% complexity classes and languages
\renewcommand{\P}{\class{P}}
\newcommand{\FP}{\class{FP}}
\newcommand{\BPP}{\class{BPP}}
\newcommand{\NP}{\class{NP}}
\newcommand{\FNP}{\class{FNP}}
\newcommand{\TFNP}{\class{TFNP}}
\newcommand{\coNP}{\class{coNP}}
\newcommand{\AM}{\class{AM}}
\newcommand{\coAM}{\class{coAM}}
\newcommand{\IP}{\class{IP}}
\newcommand{\SZK}{\class{SZK}}
\newcommand{\NISZK}{\class{NISZK}}
\newcommand{\NICZK}{\class{NICZK}}
\newcommand{\PPP}{\class{PPP}}
\newcommand{\wPPP}{\class{PWPP}}
\newcommand{\PWPP}{\wPPP}
\newcommand{\PPA}{\class{PPA}}
\newcommand{\PLS}{\class{PLS}}
\newcommand{\PPAD}{\class{PPAD}}
\newcommand{\PPADS}{\class{PPADS}}
\newcommand{\CLS}{\class{CLS}}
\newcommand{\PSPACE}{\class{PSPACE}}
\newcommand{\Ppoly}{\class{P/poly}}


%
\def\TIME{\textsc{TIME}}
\def\SPACE{\textsc{SPACE}}


\newcommand{\yes}{\ensuremath{\text{YES}}}
\newcommand{\no}{\ensuremath{\text{NO}}}

\newcommand{\Piyes}{\ensuremath{\Pi^{\yes}}}
\newcommand{\Pino}{\ensuremath{\Pi^{\no}}}


==> Local min max/headers/crypthead.tex <==
% crypto-related notation

% KEYS AND RELATED

\newcommand{\mm}[1]{\ensuremath{#1}}

\newcommand{\pp}{\mm{pp}}      % public params
\newcommand{\pk}{\mm{pk}}
\newcommand{\vk}{\mm{vk}}
\newcommand{\sk}{\mm{sk}}
\newcommand{\mpk}{\mm{mpk}}
\newcommand{\msk}{\mm{msk}}
\newcommand{\fk}{\mm{fk}}
\newcommand{\id}{id}
\newcommand{\msgspace}{\ensuremath{\mathcal{M}}}
\newcommand{\idspace}{\ensuremath{\mathcal{ID}}}

\newcommand{\concat}{\ensuremath{\|}}

% GAMES STUFF

% advantage
\newcommand{\advan}{\ensuremath{\mathbf{Adv}}}

% different attack models
\newcommand{\attack}[1]{\ensuremath{\text{#1}}}

\newcommand{\atk}{\attack{atk}} % dummy attack
\newcommand{\indcpa}{\attack{ind-cpa}}
\newcommand{\indcca}{\attack{ind-cca}}
\newcommand{\anocpa}{\attack{ano-cpa}} % anonymous
\newcommand{\anocca}{\attack{ano-cca}}
\newcommand{\sidindcpa}{\attack{sid-ind-cpa}} % selective-id
\newcommand{\aidindcpa}{\attack{aid-ind-cpa}} % adaptive-id
\newcommand{\sidindcca}{\attack{sid-ind-cca}}
\newcommand{\aidindcca}{\attack{aid-ind-cca}}
\newcommand{\euacma}{\attack{eu-acma}} % forgery: adaptive chosen-message
\newcommand{\euscma}{\attack{eu-scma}} % forgery: static chosen-message
\newcommand{\suacma}{\attack{su-acma}} % strong forgery: adaptive chosen-message
\newcommand{\suscma}{\attack{su-scma}} % strong forgery: static chosen-message

% ADVERSARIES
\newcommand{\attacker}[1]{\ensuremath{\mathcal{#1}}}

\newcommand{\Adv}{\attacker{A}}
\newcommand{\Sim}{\attacker{S}}
\newcommand{\Ora}{\attacker{O}}
\newcommand{\Inv}{\attacker{I}}
%\newcommand{\For}{\attacker{F}}

% CRYPTO SCHEMES

\newcommand{\scheme}[1]{\ensuremath{\text{#1}}}

% collision-resistant hash func family
\newcommand{\crhf}{\scheme{H}}
\newcommand{\crhfgen}{\algo{Gen}}
\newcommand{\crhfkeygen}{\algo{Keygen}}
\newcommand{\crhfhash}{\algo{Hash}}

% secret-key cryptosystem
\newcommand{\skc}{\scheme{SKC}}
\newcommand{\skcgen}{\algo{Gen}}
\newcommand{\skcenc}{\algo{Enc}} % can also use \kemenc and \kemdec
\newcommand{\skcdec}{\algo{Dec}}

% public-key cryptosystem
\newcommand{\pkc}{\scheme{PKC}}
\newcommand{\pkcsetup}{\algo{Setup}}
\newcommand{\pkcgen}{\algo{Gen}}
\newcommand{\pkcenc}{\algo{Enc}} % can also use \kemenc and \kemdec
\newcommand{\pkcdec}{\algo{Dec}}
\newcommand{\msgsp}{\mathcal{M}}

% extra deniable algorithms for pkc
\newcommand{\biden}{\scheme{BI\mbox{-}DEN}}
\newcommand{\den}{\scheme{DEN}}
\newcommand{\dengen}{\algo{DenGen}} 
\newcommand{\denenc}{\algo{DenEnc}} % can also use \kemenc and \kemdec
\newcommand{\rfake}{\algo{RecFake}}
\newcommand{\sfake}{\algo{SendFake}}

% plan ahead deniability 
\newcommand{\pden}{\scheme{PL\mbox{-}DEN}}
\newcommand{\pdenenc}{\algo{PADenEnc}} % can also use \kemenc and \kemdec
\newcommand{\prfake}{\algo{PARecFake}}
\newcommand{\psfake}{\algo{PASendFake}}

% bitranslucent sets
\newcommand{\bts}{\scheme{BTS}}
\newcommand{\btsgen}{\algo{Gen}}
\newcommand{\btsdengen}{\algo{DenGen}}
\newcommand{\sampleP}{\algo{SampleP}} 
\newcommand{\sampleU}{\algo{SampleU}} 
\newcommand{\testP}{\algo{TestP}}
\newcommand{\fakeScoins}{\algo{FakeSCoins}}
\newcommand{\fakeRcoins}{\algo{FakeRCoins}}

% digital signatures
\newcommand{\sig}{\scheme{SIG}}
\newcommand{\siggen}{\algo{Gen}}
\newcommand{\sigsign}{\algo{Sign}}
\newcommand{\sigver}{\algo{Ver}}

% key-encapsulation mechanism
\newcommand{\kem}{\scheme{KEM}}
\newcommand{\kemgen}{\algo{Gen}}
\newcommand{\kemenc}{\algo{Encaps}}
\newcommand{\kemdec}{\algo{Decaps}}

% symmetric cipher
\newcommand{\sym}{\scheme{SYM}}
\newcommand{\symenc}{\algo{E}}
\newcommand{\symdec}{\algo{D}}

% identity-based encryption
\newcommand{\ibe}{\scheme{IBE}}
\newcommand{\ibesetup}{\algo{Setup}}
\newcommand{\ibeext}{\algo{Ext}}
\newcommand{\ibeenc}{\algo{Enc}}
\newcommand{\ibedec}{\algo{Dec}}

% hierarchical IBE (as key encapsulation)
\newcommand{\hibe}{\scheme{HIBE}}
\newcommand{\hibesetup}{\algo{Setup}}
\newcommand{\hibeext}{\algo{Extract}}
\newcommand{\hibeenc}{\algo{Encaps}}
\newcommand{\hibedec}{\algo{Decaps}}

% binary tree encryption (as key encapsulation)
\newcommand{\bte}{\scheme{BTE}}
\newcommand{\btesetup}{\algo{Setup}}
\newcommand{\bteext}{\algo{Extract}}
\newcommand{\bteenc}{\algo{Encaps}}
\newcommand{\btedec}{\algo{Decaps}}

% trapdoor functions
\newcommand{\tdf}{\scheme{TDF}}
\newcommand{\tdfgen}{\algo{Gen}}
\newcommand{\tdfeval}{\algo{Eval}}
\newcommand{\tdfinv}{\algo{Invert}}
\newcommand{\tdfver}{\algo{Ver}}

% preimage samplable functions
\newcommand{\psf}{\scheme{PSF}}
\newcommand{\psfgen}{\algo{Gen}}
\newcommand{\psfsamdom}{\algo{SampleDom}}
\newcommand{\psfsampre}{\algo{SamplePre}}

% COMPLEXITY MEASURES

\newcommand{\qhash}{\ensuremath{Q_{H}}}
\newcommand{\qext}{\ensuremath{Q_{E}}}
\newcommand{\qid}{\ensuremath{Q_{\text{id}}}}
\newcommand{\qsign}{\ensuremath{Q_{\text{sign}}}}

% UC STUFF

\newcommand{\func}[1]{\ensuremath{\mathcal{F}_{#1}}\xspace}
\newcommand{\prot}[1]{\ensuremath{\mathcal{\pi}_{#1}}\xspace}
\newcommand{\exec}{\ensuremath{\text{EXEC}}}
%\newcommand{\ideal}{\ensuremath{\text{IDEAL}}}
% \Sim and \Adv are already defined above
\newcommand{\Env}{\attacker{Z}}
\newcommand{\sid}{\ensuremath{\mathsf{sid}}\xspace}
\newcommand{\ssid}{\ensuremath{\mathsf{ssid}}\xspace}
\newcommand{\command}[1]{\ensuremath{\mathsf{#1}}\xspace}


==> Local min max/headers/head.tex <==
% bring in the individual header files

\input{./headers/bbhead}
\input{./headers/calhead}
\input{./headers/lrhead}
\input{./headers/vecmathead}
\input{./headers/thmhead}
\input{./headers/comphead}
\input{./headers/latthead}
\input{./headers/crypthead}
\input{./headers/marginnotes}
\input{./headers/probhead}

\newcommand{\etal}{{et~al.}}
\mathchardef\mdash="2D % Define a "math hyphen"

% new epsilons
\newcommand{\eps}{\varepsilon}
\newcommand{\bfeps}{\boldsymbol{\varepsilon}}
\renewcommand{\epsilon}{\varepsilon}

% paragraph macro (useful because many classes redefine it}
\newcommand{\myparagraph}[1]{\paragraph{{#1}.}}

% Macros from Adeline and Damien
\newcommand{\mult}{\cdot}
\newcommand{\wn}{\omega( \sqrt{\log n})}

% macros for extLWE proof
\newcommand{\roundd}{{\mathrm{round}}}
\newcommand{\fract}{{\mathrm{frac}}}


% Macros for decision problems and such
\def\binset{\{0,1\}}
\def\bbZ{{\mathbb Z}}
\def\bbN{{\mathbb N}}
\def\bbT{{\mathbb T}}

%\def\getsr{\stackrel{\scriptscriptstyle{\$}}{\gets}}
\def\getsr{\gets}
\def\getsd{{:=}}

\newcommand{\mx}[1]{\mathbf{{#1}}}
\newcommand{\vc}[1]{\mathbf{{#1}}}
%\newcommand{\gvc}[1]{\bm{{#1}}}
\newcommand{\gvc}[1]{\vc{{#1}}}

\newcommand{\adv}{\mathrm{Adv}}

\newcommand{\zolwe}{\mathsf{binLWE}}
\def\mAh{\hat{\mx{A}}}


==> Local min max/headers/header.tex <==
%!TeX root = main.tex

%%%%%% Compact Itemize and Enumerate
\def\compactify{\itemsep=0pt \topsep=0pt \partopsep=0pt \parsep=0pt}
\let\latexusecounter=\usecounter

\newenvironment{Enumerate}
  {\def\usecounter{\compactify\latexusecounter}
   \begin{enumerate}}
  {\end{enumerate}\let\usecounter=\latexusecounter}

\newenvironment{Itemize}%
{\begin{itemize}%
\setlength{\itemsep}{0pt}%
\setlength{\topsep}{0pt}%
\setlength{\partopsep}{0 in}%
\setlength{\parskip}{0 pt}}%
{\end{itemize}}

%%%%%% General
%\def\eps{\varepsilon}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\def\floor#1{\mathop{\left\lfloor#1\right\rfloor}}
\def\ceil#1{\mathop{\left\lceil#1\right\rceil}}
\def\abs#1{\left|#1\right|}
\def\p#1{\left(#1\right)}
\def\b#1{\left[#1\right]}
\def\set#1{\left\{#1\right\}}

\newcommand{\paragr}[1]{\noindent \textbf{#1}}

%%%%%% Vectors
%\def\matr#1{\mathbf{#1}}
%\def\vect#1{\vec{#1}}

\def\norm#1{\left\|#1\right\|}
\def\snorm#1#2{\left\|#1\right\|_{#2}}

\def\zeros{\vect{0}}
\def\ones{\vect{1}}

\def\mzeros{\matr{0}}
\def\mones{\matr{1}}

%%%%%% Algorithms & Complexity
\def\poly{\mathrm{poly}}
\def\polylog{\mathrm{polylog}}

\def\TIME{\textsc{TIME}}
\def\SPACE{\textsc{SPACE}}
% \def\PSPACE{\textsc{PSPACE}}
% \def\P{\textsc{P}}
% \def\FP{\textsc{FP}}
% \def\NP{\textsc{NP}}
% \def\FNP{\textsc{FNP}}
% \def\coNP{\textsc{coNP}}
%
% \def\TFNP{\textsc{TFNP}}
% \def\PLS{\textsc{PLS}}
% \def\PPA{\textsc{PPA}}
% \def\PPP{\textsc{PPP}}
% \def\PPAD{\textsc{PPAD}}
% \def\PPADS{\textsc{PPADS}}
% \def\CLS{\textsc{CLS}}

\def\OPT{\mathrm{OPT}}
\def\cost{\mathrm{cost}}

%%%%%% Probability
%\def\Prob{\mathbb{P}}
%\def\Exp{\mathbb{E}}

%%%%%% Sets of numbers
\newcommand{\reals}{\mathbb{R}}
\newcommand{\realsp}{\mathbb{R}_{+}}
\newcommand{\realsm}{\mathbb{R}_{-}}
\newcommand{\nats}{\mathbb{N}}
\newcommand{\integer}{\mathbb{Z}}
\newcommand{\complex}{\mathbb{C}}

%%%%%% Topology
\def\Int{\mathrm{Int}}
\def\Clos{\mathrm{Clos}}

\newcommand{\diam}[2]{\mathrm{diam}_{#1}\left[ #2 \right]}

% %%%%%% Theorems
% \newtheorem{theorem}{Theorem}
% \newtheorem{inftheorem}{Informal Theorem}
% \newtheorem{proposition}{Proposition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{claim}{Claim}
% \newtheorem{corollary}{Corollary}
%
% \newtheorem{assumption}{Assumption}
% \newtheorem{definition}{Definition}
%
% % Without Numbers
% \newtheorem*{ntheorem}{Theorem}
% \newtheorem*{ninftheorem}{Informal Theorem}
% \newtheorem*{nproposition}{Proposition}
% \newtheorem*{nlemma}{Lemma}
% \newtheorem*{nclaim}{Claim}
% \newtheorem*{ncorollary}{Corollary}
%
% \newtheorem*{nassumption}{Assumption}
% \newtheorem*{ndefinition}{Definition}
%
% % Proofs
% \newenvironment{proofb}{\noindent \textit{Proof.}}{\hfill \rule{1.5ex}{1.5ex}}
%
% \newenvironment{prevproof}[2]{\noindent {\bf {Proof of {#1}~\ref{#2}:}}}{$\blacksquare$\vskip \belowdisplayskip}

%%%%%% Some Colors
%\definecolor{myC}{rgb}{0, 255, 255}
%\definecolor{myY}{rgb}{204, 204, 0}
%\definecolor{myM}{rgb}{255, 0, 255}
%\definecolor{secinhead}{RGB}{249,196,95}
%\definecolor{lgray}{gray}{0.8}
\definecolor{niceRed}{RGB}{190,38,38}
\definecolor{blueGrotto}{HTML}{059DC0}
\definecolor{royalBlue}{HTML}{057DCD}
\definecolor{navyBlueP}{HTML}{0B579C}
\definecolor{limeGreen}{HTML}{81B622}

%%%%%% Appearance
\renewcommand{\theequation}{\thesection.\arabic{equation}}

\newcommand{\chara}{\mathds{1}}


==> Local min max/headers/latthead.tex <==
% basic notation

\newcommand{\lamperp}{\Lambda^{\perp}}
\newcommand{\lam}{\Lambda}

% lattice
\newcommand{\lat}{\mathcal{L}}
% dual
\newcommand{\dual}{\mathcal{L}^{*}}
% fundamental region
\newcommand{\piped}{\mathcal{P}}
% smoothing parameter
\newcommand{\smooth}{\eta}
% smoothing w/ epsilon
\newcommand{\smootheps}{\smooth_{\epsilon}}
% ball
\newcommand{\ball}{\mathcal{B}}
% cube
\newcommand{\cube}{\mathcal{C}}
% covering radius symbol
\newcommand{\cover}{\ensuremath{\mu}}
% Gram-Schmidt
\newcommand{\gs}[1]{\ensuremath{\widetilde{#1}}}
% GS minimum
\newcommand{\gsmin}{\ensuremath{\widetilde{bl}}}
% volume operation
\DeclareMathOperator{\vol}{vol}
% Hermite normal form
\DeclareMathOperator{\hnf}{HNF}
% rank
\DeclareMathOperator{\rank}{rank}
% distance operator
\DeclareMathOperator{\dist}{dist}
% span operator
\DeclareMathOperator{\spn}{span}
% error function
\DeclareMathOperator{\erf}{erf}
% group order
\DeclareMathOperator{\ord}{ord}


% quantities that show up regularly
\newcommand{\wsln}{\ensuremath{\omega(\sqrt{\log n})}}
\newcommand{\wslm}{\ensuremath{\omega(\sqrt{\log m})}}

% support algorithms
\newcommand{\sampleZ}{\algo{Sample}\Z}
\newcommand{\sampleD}{\algo{SampleD}}
\newcommand{\tobasis}{\algo{ToBasis}}
\newcommand{\invert}{\algo{Invert}}
\newcommand{\extbasis}{\algo{ExtBasis}}
\newcommand{\extlattice}{\algo{ExtLattice}}
\newcommand{\randbasis}{\algo{RandBasis}}
\newcommand{\noisy}{\algo{Noisy}}

% problems related to lattices
\newcommand{\svp}{\problem{SVP}}
\newcommand{\gapsvp}{\problem{GapSVP}}
\newcommand{\cogapsvp}{\problem{coGapSVP}}
\newcommand{\usvp}{\problem{uSVP}}
\newcommand{\sivp}{\problem{SIVP}}
\newcommand{\gapsivp}{\problem{GapSIVP}}
\newcommand{\cvp}{\problem{CVP}}
\newcommand{\gapcvp}{\problem{GapCVP}}
\newcommand{\cvpp}{\problem{CVPP}}
\newcommand{\gapcvpp}{\problem{GapCVPP}}
\newcommand{\bdd}{\problem{BDD}}
\newcommand{\gdd}{\problem{GDD}}
\newcommand{\add}{\problem{ADD}}
\newcommand{\incgdd}{\problem{IncGDD}}
\newcommand{\incivd}{\problem{IncIVD}}
\newcommand{\crp}{\problem{CRP}}
\newcommand{\gapcrp}{\problem{GapCRP}}
\newcommand{\dgs}{\problem{DGS}}
% avg-case stuff
\newcommand{\sis}{\problem{SIS}}
\newcommand{\isis}{\problem{ISIS}}
\newcommand{\ilwe}{\problem{ILWE}}
\newcommand{\lwe}{\problem{LWE}}
\newcommand{\rlwe}{\problem{RLWE}}
\newcommand{\declwe}{\problem{WDLWE}}
\newcommand{\extlwe}{\problem{extLWE}}
\newcommand{\dlwe}{\problem{DLWE}}
\newcommand{\lpn}{\problem{LPN}}
\newcommand{\Psibar}{\ensuremath{\bar{\Psi}}}


==> Local min max/headers/lrhead.tex <==
% "left-right" pairs of symbols

%% NOTE: this requires \usepackage{mathtools} in the document preamble

% inner product
\DeclarePairedDelimiter\inner{\langle}{\rangle}
% absolute value
%\DeclarePairedDelimiter\abs{\lvert}{\rvert}
% a set
%\DeclarePairedDelimiter\set{\{}{\}}
% parens
\DeclarePairedDelimiter\parens{(}{)}
% tuple, alias for parens
\DeclarePairedDelimiter\tuple{(}{)}
% square brackets
\DeclarePairedDelimiter\bracks{[}{]}
% rounding off
\DeclarePairedDelimiter\round{\lfloor}{\rceil}
% floor function
%\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
% ceiling function
%\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
% length of some vector, element
%\DeclarePairedDelimiter\norm{\lVert}{\rVert}
%\DeclarePairedDelimiter\length{\lVert}{\rVert}
% "lifting" of a residue class
\DeclarePairedDelimiter\lift{\llbracket}{\rrbracket}


==> Local min max/headers/marginnotes.tex <==
% MARGIN NOTES

\newif\ifnotes\notestrue
% \newif\ifnotes\notesfalse


\ifnotes
\usepackage{color}
\definecolor{mygrey}{gray}{0.50}
%\newcommand{\notename}[2]{{\textcolor{mygrey}{\footnotesize{\bf (#1:} {#2}{\bf
%) }}}}
\newcommand{\notename}[2]{{\textcolor{red}{\footnotesize{\bf (#1:} {#2}{\bf
) }}}}
\newcommand{\noteswarning}{{\begin{center} {\Large WARNING: NOTES ON}\end{center}}}

\else

\newcommand{\notename}[2]{{}}
\newcommand{\noteswarning}{{}}

\fi

\newcommand{\cnote}[1]{{\notename{Costis}{#1}}}
\newcommand{\snote}[1]{{\notename{Stratis}{#1}}}
\newcommand{\mnote}[1]{{\notename{Manolis}{#1}}}

==> Local min max/headers/packages.tex <==
%!TeX root = main.tex
%!TeX root = ppp.tex

\linespread{1.06}
\usepackage[sc]{mathpazo}

\usepackage[margin=1in]{geometry}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[compact]{titlesec}
\usepackage[usenames,dvipsnames]{xcolor}

%% These have been added at the request of the MIT Libraries, because
%% some PDF conversions mess up the ligatures.  -LB, 1/22/2014
\usepackage{cmap}
\usepackage[T1]{fontenc}
\usepackage{bm}
\pagestyle{plain}

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsbsy}
\usepackage{amsthm}
\usepackage{dsfont}

% g
\usepackage{mathtools}
\usepackage{xspace}
%\usepackage[amsmath,thmmarks,hyperref]{ntheorem}

\usepackage{graphicx, ucs}

\usepackage{subcaption}
\usepackage{rotating}
\usepackage{float}
\usepackage{tikz}

\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{listings}

\usepackage{enumitem}
\usepackage{hyperref}
\hypersetup{
  colorlinks = true,
  urlcolor = {blueGrotto},
  linkcolor = {royalBlue},
  citecolor = {navyBlueP}
}
\usepackage{multirow}
\usepackage{array}

\usepackage{accents}

\usepackage[outline]{contour}% http://ctan.org/pkg/contour

\usepackage[%
linewidth=3pt,
linecolor=gray,
middlelinecolor= black,
middlelinewidth=0.4pt,
roundcorner=1pt,
topline = false,
rightline = false,
bottomline = false,
rightmargin=0pt,
skipabove=0pt,
skipbelow=0pt,
leftmargin=0pt,
innerleftmargin=4pt,
innerrightmargin=0pt,
innertopmargin=0pt,
innerbottommargin=0pt,
]{mdframed}

\usepackage{chngcntr}
\usepackage{soul}
\usepackage{arydshln}


==> Local min max/headers/probhead.tex <==
% macros for probability distributions
\newcommand{\normal}{\mathcal{N}}
\newcommand{\Bernoulli}{\mathcal{B}}
\newcommand{\geometric}{\mathcal{G}}

% Expectations
\DeclareMathOperator*{\Exp}{{\mathbb{E}}}
\DeclareMathOperator*{\Prob}{{\mathbb{P}}}
\DeclareMathOperator*{\Cov}{{\mathrm{Cov}}}
\DeclareMathOperator*{\Var}{\mathrm{Var}}
\DeclareMathOperator*{\KL}{\mathrm{D}_{\mathrm{KL}}}
\DeclareMathOperator*{\TV}{\mathrm{d}_{\mathrm{TV}}}


==> Local min max/headers/thmhead.tex <==
\theoremstyle{plain}            % following are "theorem" style
\newtheorem{theorem}{Theorem}[section]
\newtheorem{inftheorem}{Informal Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{techlemma}[theorem]{Technical Lemma}

\newtheorem{maintheorem}{Main Theorem}

\theoremstyle{definition}       % following are def style
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{remark}           % following are remark style
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{note}[theorem]{Note}

% equation numbering style
\numberwithin{equation}{section}

% without Numbers
\newtheorem*{ntheorem}{Theorem}
\newtheorem*{ninftheorem}{Informal Theorem}
\newtheorem*{nproposition}{Proposition}
\newtheorem*{nlemma}{Lemma}
\newtheorem*{nclaim}{Claim}
\newtheorem*{ncorollary}{Corollary}
\newtheorem*{nassumption}{Assumption}
\newtheorem*{ndefinition}{Definition}

% Proofs
\newenvironment{proofb}[1]{\noindent \textit{Proof #1.}}{\hfill \rule{1.5ex}{1.5ex}}

\newenvironment{prevproof}[2]{\noindent {\bf {Proof of
{#1}~\ref{#2}:}}}{$\blacksquare$\vskip \belowdisplayskip}

% Problem Environment
\contourlength{0.1pt}
\contournumber{10}

\newenvironment{nproblem}[1][\unskip]{%
\medskip
\begin{mdframed}
\noindent
\contour{black}{\underline{$#1$.}} \\
\noindent}
{\end{mdframed}}


==> Local min max/headers/vecmathead.tex <==
% macros for matrices and vectors
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\newcommand{\matr}[1]{\boldsymbol{#1}}

\DeclareMathOperator*{\diag}{\mathrm{diag}}

\newcommand{\matA}{\ensuremath{\boldsymbol{A}}}
\newcommand{\matB}{\ensuremath{\boldsymbol{B}}}
\newcommand{\matC}{\ensuremath{\boldsymbol{C}}}
\newcommand{\matD}{\ensuremath{\boldsymbol{D}}}
\newcommand{\matE}{\ensuremath{\boldsymbol{E}}}
\newcommand{\matF}{\ensuremath{\boldsymbol{F}}}
\newcommand{\matG}{\ensuremath{\boldsymbol{G}}}
\newcommand{\matH}{\ensuremath{\boldsymbol{H}}}
\newcommand{\matI}{\ensuremath{\boldsymbol{I}}}
\newcommand{\matJ}{\ensuremath{\boldsymbol{J}}}
\newcommand{\matK}{\ensuremath{\boldsymbol{K}}}
\newcommand{\matL}{\ensuremath{\boldsymbol{L}}}
\newcommand{\matM}{\ensuremath{\boldsymbol{M}}}
\newcommand{\matN}{\ensuremath{\boldsymbol{N}}}
\newcommand{\matP}{\ensuremath{\boldsymbol{P}}}
\newcommand{\matQ}{\ensuremath{\boldsymbol{Q}}}
\newcommand{\matR}{\ensuremath{\boldsymbol{R}}}
\newcommand{\matS}{\ensuremath{\boldsymbol{S}}}
\newcommand{\matT}{\ensuremath{\boldsymbol{T}}}
\newcommand{\matU}{\ensuremath{\boldsymbol{U}}}
\newcommand{\matV}{\ensuremath{\boldsymbol{V}}}
\newcommand{\matW}{\ensuremath{\boldsymbol{W}}}
\newcommand{\matX}{\ensuremath{\boldsymbol{X}}}
\newcommand{\matY}{\ensuremath{\boldsymbol{Y}}}
\newcommand{\matZ}{\ensuremath{\boldsymbol{Z}}}
\newcommand{\matzero}{\ensuremath{\boldsymbol{0}}}

\newcommand{\veca}{\ensuremath{\boldsymbol{a}}}
\newcommand{\vecb}{\ensuremath{\boldsymbol{b}}}
\newcommand{\vecc}{\ensuremath{\boldsymbol{c}}}
\newcommand{\vecd}{\ensuremath{\boldsymbol{d}}}
\newcommand{\vece}{\ensuremath{\boldsymbol{e}}}
\newcommand{\vecf}{\ensuremath{\boldsymbol{f}}}
\newcommand{\vecg}{\ensuremath{\boldsymbol{g}}}
\newcommand{\vech}{\ensuremath{\boldsymbol{h}}}
\newcommand{\veck}{\ensuremath{\boldsymbol{k}}}
\newcommand{\vecm}{\ensuremath{\boldsymbol{m}}}
\newcommand{\vecp}{\ensuremath{\boldsymbol{p}}}
\newcommand{\vecq}{\ensuremath{\boldsymbol{q}}}
\newcommand{\vecr}{\ensuremath{\boldsymbol{r}}}
\newcommand{\vecs}{\ensuremath{\boldsymbol{s}}}
\newcommand{\vect}{\ensuremath{\boldsymbol{t}}}
\newcommand{\vecu}{\ensuremath{\boldsymbol{u}}}
\newcommand{\vecv}{\ensuremath{\boldsymbol{v}}}
\newcommand{\vecw}{\ensuremath{\boldsymbol{w}}}
\newcommand{\vecx}{\ensuremath{\boldsymbol{x}}}
\newcommand{\vecy}{\ensuremath{\boldsymbol{y}}}
\newcommand{\vecz}{\ensuremath{\boldsymbol{z}}}
\newcommand{\veczero}{\ensuremath{\boldsymbol{0}}}

